Remember Me, Refine Me: A Dynamic Procedural Memory Framework for Experience-Driven Agent Evolution

Procedural memory enables large language model (LLM) agents to internalize "how-to" knowledge, theoretically reducing redundant trial-and-error. However, existing frameworks predominantly suffer from a "passive accumulation" paradigm, treating memory as a static append-only archive. To bridge the gap between static storage and dynamic reasoning, we propose $\textbf{ReMe}$ ($\textit{Remember Me, Refine Me}$), a comprehensive framework for experience-driven agent evolution. ReMe innovates across the memory lifecycle via three mechanisms: 1) $\textit{multi-faceted distillation}$, which extracts fine-grained experiences by recognizing success patterns, analyzing failure triggers and generating comparative insights; 2) $\textit{context-adaptive reuse}$, which tailors historical insights to new contexts via scenario-aware indexing; and 3) $\textit{utility-based refinement}$, which autonomously adds valid memories and prunes outdated ones to maintain a compact, high-quality experience pool. Extensive experiments on BFCL-V3 and AppWorld demonstrate that ReMe establishes a new state-of-the-art in agent memory system. Crucially, we observe a significant memory-scaling effect: Qwen3-8B equipped with ReMe outperforms larger, memoryless Qwen3-14B, suggesting that self-evolving memory provides a computation-efficient pathway for lifelong learning. We release our code and the $\texttt{reme.library}$ dataset to facilitate further research.

==> sections/abstract_origin.tex <==
\begin{abstract}
Procedural memory is fundamental to large language model (LLM) agents, accumulating and reusing past experiences for enhanced decision-making. 
However, existing memory-driven systems often store coarse-grained, trajectory-level experiences, which potentially introduce redundancy or interference in agent reasoning. 
Motivated by the need for finer granularity, we propose a novel memory framework called {\ours} that distills keypoint-level experiences from historical interactions, each capturing a critical decision step that directly influences task outcomes. 
To ensure long-term memory quality, {\ours} employs an LLM-independent, utility-based refinement mechanism that incorporates only reliable experiences and prunes ineffective ones. 
Our framework enables agents to leverage prior knowledge effectively, avoid blind exploration, and maintain a high-quality, dynamic experience pool that evolves with their improving capabilities. 
Experiments on BFCL-V3 and AppWorld show that {\ours} significantly boosts the agent's task-solving ability, yielding average absolute performance gains of 10.65\% Avg@4 and 10.53\% Pass@4 compared to the naive Qwen3-8B baseline. 
Ablation studies confirm the advantage of fine-grained experience collection and further reveal that combining robust experience refinement with failure-aware reflection promisingly strengthens the agent experience-driven inference. 
\end{abstract}




==> sections/abstract_v1.tex <==
\begin{abstract}
Procedural memory enables agents to internalize past experiences for enhanced decision-making, yet existing systems predominantly adopt a passive ``store-and-retrieve'' paradigm.
This approach inevitably leads to \textit{memory degradation}, where the accumulation of redundant or obsolete interactions dilutes critical reasoning signals and hinders adaptation in non-stationary environments.
To address this, we propose \textbf{\ours} (\textit{Remember Me, Refine Me}), a dynamic framework that shifts the focus from raw retention to \textbf{feedback-driven experience evolution}.
Instead of indiscriminately archiving interactions, {\ours} employs a \textbf{contrastive distillation strategy}, analyzing the divergence between successful and failed attempts to extract high-value causal insights.
Crucially, to maintain memory vitality, we introduce a \textbf{utility-based refinement mechanism} that autonomously reinforces validated strategies while pruning ineffective entries, coupled with a \textbf{failure-aware reflection} protocol to adapt memories during distinct task failures.
Experiments on BFCL-V3 and AppWorld demonstrate that {\ours} establishes a new state-of-the-art, achieving average gains of 10.65\% in Avg@4.
Notably, our framework enables a Qwen3-8B agent to outperform a parameter-heavier Qwen3-14B baseline, highlighting that self-evolving memory offers a compute-efficient pathway to transcend model scaling limitations.
\end{abstract}

==> sections/abstract_v2.tex <==

\begin{abstract}
Procedural memory enables autonomous agents to internalize ``how-to'' knowledge, theoretically reducing redundant trial-and-error. 
However, existing frameworks predominantly suffer from a ``passive accumulation'' paradigm, treating memory as a static
append-only archive, storing raw, trajectory-level
interactions.
To bridge the gap between static storage and dynamic reasoning, we propose \textbf{\ours} (\textit{Remember Me, Refine Me}), a comprehensive framework for experience-driven agent evolution. 
\textbf{\ours} innovates across the memory lifecycle via three mechanisms: (1) \textbf{contrastive distillation}, which extracts high-fidelity causal decision points by analyzing the divergence between successful and failed attempts; (2) \textbf{context-adaptive reuse}, which employs reranking, rewriting, and failure-aware reflection to tailor historical insights to new contexts; and (3) \textbf{utility-based refinement}, which autonomously prunes obsolete entries to maintain a compact, high-value memory pool. 
Extensive experiments on BFCL-V3 and AppWorld benchmarks demonstrate that \textbf{\ours} establishes a new state-of-the-art. 
Crucially, we observe a significant \textbf{memory-scaling effect}: a Qwen3-8B model equipped with \ours outperforms a parameter-heavier Qwen3-14B baseline, suggesting that self-evolving memory offers a computation-efficient pathway for lifelong learning. 
We release our code and the \texttt{reme.library} dataset to facilitate further research.
\end{abstract}

==> sections/introduction_origin.tex <==
\section{Introduction}
The emergence of large language model (LLM) agents marks a new paradigm~\citep{cheng2024exploring,tao2024survey,gao2025survey,fang2025comprehensive}, delivering significant improvements over static models in complex, dynamic task environments. 
Memory serves as a crucial component in prompting agent test-time self-evolution~\citep{zhang2025survey}, which provides a substrate for accumulating, organizing, and reusing past knowledge without retraining the base model~\citep{xu2025mem,tang2025agentkb}. 
% Consequently, how to design an effective memory system for agents has garnered increasing attention. 
Among memory paradigms, procedural memory is particularly attractive for agents, as it gathers high-quality problem-solving experiences from historical interaction trajectories~\citep{wang2025mirix,fang2025memp}. 
These experiences can be leveraged to guide agent decision-making in new tasks, thereby reducing redundant trial-and-error and avoiding local optima~\citep{chen2025swe} (as shown in Figure~\ref{fig:example}). 

Existing memory systems predominantly store complete trajectories as experiences~\citep{zheng2023synapse,hu2024hiagent} or summarize structured workflows~\citep{tang2025agentkb,chen2025swe,liu-etal-2025-contextual} corresponding to entire trajectories. 
However, these approaches often overlook the importance of choosing an appropriate level of granularity, since coarse-grained trajectory-level experiences may contain irrelevant information that can mislead agents into making erroneous decisions in new tasks. 
This motivates us to explore the potential of fine-grained keypoint-level experiences, which distill critical steps that influence task outcomes. 
Moreover, as task distribution shifts and agent self-improves over time, stored experiences may become inapplicable or inefficient~\citep{xiong2025memory}. 
Consequently, an effective experience refinement mechanism is essential to maintain memory quality for long-term agent performance. 
While prior works have investigated memory management strategies for LLM agents~\citep{chhikara2025mem0,yan2025memory}, they mainly require prompting or fine-tuning LLMs to select memory operations, failing to establish LLM-independent, quantitative criteria for experience addition and deletion.

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/example.pdf}
    \caption{Example of how agents complete one stock trading task with and without past experience.}\label{fig:example}
\end{figure*}

In this work, we propose {\ours}, a procedural memory framework that focuses on keypoint-level experience collection for LLM agents. 
Our goal is to maintain a dynamic, high-quality experience pool that enables agents to achieve performance improvement over time. 
Specifically, {\ours} distills key steps from past execution trajectories into structured, reusable experiences, including success pattern recognition, failure analysis and comparative insights. 
When faced with a new task, {\ours} recalls relevant experiences, guiding the agent to avoid blind exploration and allowing it to leverage prior knowledge for enhanced problem-solving capability. 
{\ours} further introduces an experience refinement strategy to maintain the long-term quality of the experience pool that only incorporates new experiences from successful trajectories for reliability and periodically removes ineffective experiences based on their utility. 


Experiments on BFCL-V3 and AppWorld benchmarks show that {\ours} significantly enhances agent performance, with Qwen3-8B improving Avg@4 from 40.33\% to 46.33\% on BFCL-V3 and from 14.97\% to 30.75\% on AppWorld. % on average?
Our ablation studies reveal that fine-grained keypoint-level experiences bring greater performance gains than coarse-grained trajectory-level ones. 
Also, {\ours} significantly enhances experience pool resilience in dynamic environments through our designed robust experience refinement strategy. 
Moreover, lessons from failure trajectories support agent self-reflection, facilitating the exploration on viable solutions.
Overall, we summarize the key contributions as follows: 
\begin{itemize}[leftmargin=12pt,topsep=2pt,itemsep=-2pt]
    \item We present {\ours}, a simple yet effective memory framework that leverages procedural memory (i.e., experience) to continuously enhance agent performance over time.
    \item We validate the advantage of collecting experiences at a fine-grained level over coarse-grained approaches. Our experience refinement mechanism further enables a self‑evolving experience pool that guides long‑term agent behavior.
    \item Experimental results reveal that {\ours} achieves superior agent performance compared to other baselines. Moreover, extensive ablation studies on memory design provide actionable insights for experience-driven agent evolution.
\end{itemize}




==> sections/introduction_v1.tex <==

\section{Introduction}

The transition from static language models to autonomous agents marks a pivotal shift in artificial intelligence, enabling systems to handle complex, dynamic tasks through iterative reasoning and tool use~\citep{cheng2024exploring,tao2024survey,gao2025survey,fang2025comprehensive}. 
To facilitate continuous improvement without expensive parameter retraining, \textbf{procedural memory}—which internalizes ``how-to'' knowledge from past interactions—has emerged as a critical substrate for agent evolution~\citep{zhang2025survey,xu2025mem}. 
By accumulating high-quality problem-solving experiences, agents can leverage prior successes to navigate novel scenarios, theoretically reducing redundant trial-and-error and circumventing local optima~\citep{wang2025mirix,chen2025swe} (as shown in Figure~\ref{fig:example}).

However, despite the promise of memory-augmented agents, current frameworks predominantly suffer from a \textbf{``passive accumulation''} paradigm. 
Prevailing approaches typically treat memory as a static append-only archive, storing raw, trajectory-level interactions~\citep{zheng2023synapse,hu2024hiagent} or generalized workflows~\citep{tang2025agentkb,liu-etal-2025-contextual}. 
This introduces two fundamental limitations. 
First, the \textbf{granularity mismatch}: retaining entire trajectories introduces significant contextual noise (e.g., irrelevant observations), which dilutes the agent's attention on critical reasoning logic during retrieval. 
Second, the \textbf{lack of evolution}: agents operate in non-stationary environments where task distributions shift and their own capabilities improve. Without a mechanism to prune obsolete or ineffective entries, the memory pool inevitably degrades into a mixture of valid insights and ``toxic'' noise, leading to negative transfer and hallucinations~\citep{xiong2025memory}.

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/example.pdf}
    \caption{Example of how agents complete one stock trading task with and without past experience.}\label{fig:example}
\end{figure*}

To address these challenges, we propose \textbf{\ours} (\textit{Remember Me, Refine Me}), a dynamic framework that shifts the paradigm from passive storage to \textbf{feedback-driven experience evolution}. 
Instead of indiscriminately archiving trajectories, {\ours} employs a \textbf{contrastive distillation strategy}. By analyzing the divergence between successful and failed attempts, the system isolates the \textbf{pivotal decision points}—the specific strategic moves that differentiate high-quality outcomes from suboptimal ones—thereby maximizing the signal-to-noise ratio of stored knowledge.
Furthermore, to combat memory degradation, {\ours} introduces a \textbf{utility-based evolutionary mechanism}. 
Treating the memory pool as a living ecosystem, our framework quantitatively tracks the utility of each experience during reuse. It autonomously reinforces validated strategies while pruning entries that fail to contribute to task success, ensuring the memory pool continuously adapts to changes in the problem and the agent's development.

Our extensive experiments on BFCL-V3 and AppWorld benchmarks demonstrate that {\ours} establishes a new state-of-the-art for memory-augmented agents. 
Most notably, our results reveal that memory quality can substitute for model scale: \textbf{{\ours} enables a Qwen3-8B model to outperform a parameter-heavier Qwen3-14B baseline (without memory)}, achieving average gains of 10.65\% in Avg@4. 
These findings suggest that a self-evolving memory mechanism offers a computationally efficient pathway for agent evolution, narrowing the gap between small and large models through strategic experience management.

In summary, our contributions are as follows:
\begin{itemize}[leftmargin=12pt,topsep=2pt,itemsep=-2pt]
    \item We propose \textbf{\ours}, a dynamic framework that evolves procedural memory through \textbf{contrastive experience distillation}, extracting keypoint-level insights to resolve the granularity mismatch inherent in trajectory-based approaches.
    \item We introduce a \textbf{utility-based evolutionary mechanism} that establishes a quantitative feedback loop for memory management, enabling the agent to autonomously maintain a high-quality, adaptive memory pool by pruning ineffective entries.
    \item We design a context-adaptive reuse strategy that incorporates \textbf{failure-aware reflection}, allowing agents to dynamically adjust their reasoning paths when historical experiences do not perfectly align with new tasks.
    \item Empirical results confirm that {\ours} significantly enhances agent performance, allowing smaller models to surpass larger baselines and demonstrating a scalable approach to lifelong agent learning.
\end{itemize}


==> sections/introduction_v2.tex <==
\section{Introduction}

The transition from static language models to autonomous agents marks a pivotal shift in artificial intelligence, enabling systems to handle complex, dynamic tasks through iterative reasoning and tool use~\citep{cheng2024exploring,tao2024survey,gao2025survey,fang2025comprehensive}. 
To facilitate continuous improvement without expensive parameter retraining, \textbf{procedural memory}—which internalizes ``how-to'' knowledge from past interactions—has emerged as a critical substrate for agent evolution~\citep{zhang2025survey,xu2025mem}. 
By accumulating high-quality problem-solving experiences, agents can leverage prior successes to navigate novel scenarios, theoretically reducing redundant trial-and-error and circumventing local optima~\citep{wang2025mirix,chen2025swe}.

To bridge the gap between static storage and dynamic reasoning, an ideal procedural memory system must function not merely as a database, but as an evolving cognitive substrate satisfying three core criteria:
(1) \textbf{High-Fidelity Extraction}: The system should distill generalized principles from noisy execution traces, ensuring that stored memories represent high-quality causal knowledge rather than raw observations.
(2) \textbf{Context-Adaptive Utilization}: Retrieved memories must be dynamically adapted to the nuances of the current task, maximizing their utility in novel scenarios.
(3) \textbf{Timely Evolution}: The memory pool must maintain its vitality through continuous updates, autonomously reinforcing effective strategies while purging obsolete entries to prevent degradation over time.

However, despite the promise of memory-augmented agents, current frameworks often fall short of these ideals, predominantly suffering from a \textbf{``passive accumulation''} paradigm. 
Prevailing approaches typically treat memory as a static append-only archive, storing raw, trajectory-level interactions~\citep{zheng2023synapse,hu2024hiagent} or generalized workflows~\citep{tang2025agentkb,liu-etal-2025-contextual}. 
This introduces fundamental limitations:
\textit{Abstraction Deficit}, where retaining entire trajectories introduces instance-specific noise that dilutes critical reasoning signals, preventing the agent from grasping the core logic; % Modified here
\textit{Rigid Retrieval}, where fetched experiences are applied without adaptation, leading to failures in slightly shifted contexts;
and crucially, \textit{Lack of Maintenance}, where the absence of timely update strategies causes the memory pool to degrade into a mixture of valid insights and toxic noise~\citep{xiong2025memory}.
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figures/example.pdf}
    \caption{Example of how agents complete one stock trading task with and without past experience.}\label{fig:example}
\end{figure*}

To address these challenges, we propose \textbf{\ours} (\textit{Remember Me, Refine Me}), a dynamic framework that shifts the paradigm from passive storage to \textbf{feedback-driven experience evolution}. 
We systematically innovate across the memory lifecycle to meet the criteria of an ideal system.
First, for \textit{High-Fidelity Extraction}, {\ours} employs a \textbf{contrastive distillation strategy}. By analyzing the divergence between successful and failed attempts, the system isolates \textbf{pivotal decision points}—the specific strategic moves that differentiate high-quality outcomes from suboptimal ones—thereby maximizing the signal-to-noise ratio.
Second, for \textit{Context-Adaptive Utilization}, we design a comprehensive reuse pipeline. Beyond simple retrieval, this module employs \textbf{reranking and adaptive rewriting} to tailor historical insights to the specific constraints of new tasks, supplemented by a \textbf{failure-aware reflection} protocol to dynamically adjust reasoning paths when direct application proves insufficient.
Finally, for \textit{Timely Evolution}, {\ours} implements a \textbf{utility-based refinement mechanism}. Treating the memory pool as a living ecosystem, our framework tracks the utility of each experience during reuse, autonomously pruning entries that fail to contribute to task success to maintain a compact and highly effective memory state.

Our extensive experiments on BFCL-V3 and AppWorld benchmarks demonstrate that {\ours} establishes a new state-of-the-art for memory-augmented agents. 
Most notably, our results reveal that memory quality can substitute for model scale: \textbf{{\ours} enables a Qwen3-8B model to outperform a parameter-heavier Qwen3-14B baseline (without memory)}, achieving average gains of 10.65\% in Avg@4. 
These findings suggest that a self-evolving memory mechanism offers a computationally efficient pathway for lifelong agent learning.

In summary, our contributions are as follows:
\begin{itemize}[leftmargin=12pt,topsep=2pt,itemsep=2pt]
    \item We propose \textbf{\ours}, a comprehensive framework for agent evolution that integrates contrastive experience distillation, context-adaptive reuse, and utility-driven refinement. This closes the loop of procedural memory, resolving the ``passive accumulation'' dilemma by enabling agents to autonomously distill, adapt, and maintain high-quality reasoning patterns.
    
    \item We release \textbf{\texttt{reme.library}}, a fine-grained procedural memory dataset constructed from diverse agentic tasks. Containing structured success patterns and failure lessons, this library serves as a valuable resource for the community to study procedure memory and optimize memory-augmented agents.
    
    \item Extensive experiments show that {\ours} significantly enhances agent performance across diverse benchmarks. Crucially, we demonstrate a \textbf{memory-scaling effect}, where smaller models equipped with {\ours} surpass larger baselines, validating our framework as a computationally efficient pathway for lifelong agent learning.
\end{itemize}

